Optimizing SLAM Evaluation Footprint Through Dynamic Range Coverage Analysis of Datasets

Simultaneous Localization and Mapping (SLAM) is considered an ever-evolving problem due to its usage in many applications. Evaluation of SLAM is done typically using publicly available datasets which are increasing in number and the level of difficulty. Each dataset provides a certain level of dynamic range coverage that is a key aspect of measuring the robustness and resilience of SLAM. In this paper, we provide a systematic analysis of the dynamic range coverage of datasets based on a number of characterization metrics, and our analysis shows a huge level of redundancy within and between datasets. Subsequently, we propose a dynamic programming (DP) algorithm for eliminating the redundancy in the evaluation process of SLAM by selecting a subset of sequences that matches a single or multiple dynamic range coverage objectives. It is shown that, with the help of dataset characterization and DP selection algorithm, a reduction in the evaluation effort can be achieved while maintaining the same level of coverage. We also study how the evaluation process of a real-world SLAM system can be optimized utilizing the method proposed.

==> figs/ATE_analysis.tex <==
\begin{figure}[!tp]
     \centering
         \includegraphics[width=\columnwidth]{../../project/Coverage_Analysis/out_figs/ATE_vs_coverage.png}
        \caption{ATE Properties after using the reduced evaluation set for ORB-SLAM3 (left) and VINS-Mono (right)}
        \label{fig:ATE_results}
\end{figure}

==> figs/ATE_rand_test.tex <==
% Correlation plots
\begin{figure}[!tp]
     \centering
     \begin{subfigure}[b]{0.48\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{img/ORBSLAM3.png}
         \caption{}
     \end{subfigure}
     \hfill   
     \begin{subfigure}[b]{0.48\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{img/VINSMONO.png}
         \caption{}
     \end{subfigure}
        \caption{Wasserstine Distance of randomly selected sub-set vs. DP-Selected Subset, compared to the full TUM-VI dataset ATE distribution of (a) ORB-SLAM3 and (b) VINS-Mono}
        \label{fig:ATE_rand_fig}
\end{figure}

==> figs/DP_desc.tex <==
\begin{figure}[!tp]
     \centering
         \includegraphics[width=\columnwidth]{img/DP_BD.png}
        \caption{A Flowchart of the Tabulation-based Dynamic Programming Optimization}
        \label{fig:DP_BD}
\end{figure}

==> figs/agg_result_main.tex <==
% Correlation plots
\begin{figure*}[!htb]
     \centering
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Coverage_Analysis/out_data/General_CoverageCost.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Coverage_Analysis/out_data/General_EffectiveCoveragePercentage.png}
     \end{subfigure}  
     \hfill     
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Coverage_Analysis/out_data/General_weightedCoverageCost.png}
     \end{subfigure}     
	 \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Coverage_Analysis/out_data/General_SeqToFullCoverage.png}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Coverage_Analysis/out_data/Inertial_CoverageCost.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Coverage_Analysis/out_data/Inertial_EffectiveCoveragePercentage.png}
     \end{subfigure}   
     \hfill     
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Coverage_Analysis/out_data/Inertial_weightedCoverageCost.png}
     \end{subfigure}    
	 \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Coverage_Analysis/out_data/Inertial_SeqToFullCoverage.png}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Coverage_Analysis/out_data/Visual_CoverageCost.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Coverage_Analysis/out_data/Visual_EffectiveCoveragePercentage.png}
     \end{subfigure}   
     \hfill     
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Coverage_Analysis/out_data/Visual_weightedCoverageCost.png}
     \end{subfigure}    
	 \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Coverage_Analysis/out_data/Visual_SeqToFullCoverage.png}
     \end{subfigure}
        \caption{Aggregated Coverage and Dynamic Range Analysis Results. Each row represents a characterization metric category which are: general metrics, inertial metrics, and visual metrics respectively. Columns represent the average coverage cost, the effective coverage percentage, the weighted average cost per coverage percentage, and the no. of sequences required to reach full coverage.}
        \label{fig:agg_results}
\end{figure*}

==> figs/agg_results.tex <==
% Correlation plots
\begin{figure}[!tp]
     \centering
     \begin{subfigure}[b]{0.31\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Coverage_Analysis/out_data/General_CoverageCost.png}
     \end{subfigure}
     \hfill   
     \begin{subfigure}[b]{0.31\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Coverage_Analysis/out_data/Inertial_CoverageCost.png}
     \end{subfigure}
     \hfill 
     \begin{subfigure}[b]{0.31\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Coverage_Analysis/out_data/Visual_CoverageCost.png}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{0.31\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Coverage_Analysis/out_data/General_EffectiveCoveragePercentage.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[b]{0.31\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Coverage_Analysis/out_data/Inertial_EffectiveCoveragePercentage.png}
     \end{subfigure}  
     \hfill     
     \begin{subfigure}[b]{0.31\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Coverage_Analysis/out_data/Visual_EffectiveCoveragePercentage.png}
     \end{subfigure} 
     \\
     \begin{subfigure}[b]{0.31\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Coverage_Analysis/out_data/General_SeqToFullCoverage.png}
     \end{subfigure}
	 \hfill
     \begin{subfigure}[b]{0.31\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Coverage_Analysis/out_data/Inertial_SeqToFullCoverage.png}
     \end{subfigure}
	 \hfill
     \begin{subfigure}[b]{0.31\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Coverage_Analysis/out_data/Visual_SeqToFullCoverage.png}
     \end{subfigure}
        \caption{Aggregated Coverage and Dynamic Range Analysis Results. Each column represents a characterization metric category which are: general metrics, inertial metrics, and visual metrics respectively. Rows represent the average coverage cost, the effective coverage percentage, and the no. of sequences required to reach full coverage.}
        \label{fig:agg_results}
\end{figure}

==> figs/char_results.tex <==
\begin{figure}[t!]
     \centering
     \begin{subfigure}[b]{0.32\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Framework/out_data/agg_figs/KDEplot_figs/KDE_FAST_DIST_AVG.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[b]{0.32\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Framework/out_data/agg_figs/KDEplot_figs/KDE_REVISIT_SCORE.png}
     \end{subfigure}  
     \hfill     
     \begin{subfigure}[b]{0.32\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Framework/out_data/agg_figs/KDEplot_figs/KDE_BLUR_PERCENT.png}
     \end{subfigure}     
     \\
     \begin{subfigure}[b]{0.32\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Framework/out_data/agg_figs/raincloud_figs/raincloud_FAST_DIST_AVG.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[b]{0.32\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Framework/out_data/agg_figs/raincloud_figs/raincloud_REVISIT_SCORE.png}
     \end{subfigure}  
     \hfill     
     \begin{subfigure}[b]{0.32\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{../../project/Framework/out_data/agg_figs/raincloud_figs/raincloud_BLUR_PERCENT.png}
     \end{subfigure}      
     
        \caption{Sample Characterization Results of SLAM Datasets}
        \label{fig:char_results}
\end{figure}

==> figs/covCost_LCO.tex <==
% Correlation plots
\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.31\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{../../project/Coverage_Analysis/out_data/General_LCO_covEfficiency.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[b]{0.62\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{../../project/Coverage_Analysis/out_data/Inertial_LCO_covEfficiency.png}
     \end{subfigure}      
	 \\
     \begin{subfigure}[b]{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{../../project/Coverage_Analysis/out_data/Visual_LCO_covEfficiency.png}
     \end{subfigure}
     \hfill
        \caption{Coverage Cost - Least Cost}
        \label{fig:covCost_LCO}
\end{figure}

==> figs/covCost_LEO.tex <==
% Correlation plots
\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.31\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{../../project/Coverage_Analysis/out_data/General_LEO_covEfficiency.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[b]{0.62\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{../../project/Coverage_Analysis/out_data/Inertial_LEO_covEfficiency.png}
     \end{subfigure}      
	 \\
     \begin{subfigure}[b]{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{../../project/Coverage_Analysis/out_data/Visual_LEO_covEfficiency.png}
     \end{subfigure}
     \hfill
        \caption{Coverage Cost - Least Experiments}
        \label{fig:covCost_LEO}
\end{figure}

==> figs/covDR_LCO.tex <==
% Correlation plots
\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.31\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{../../project/Coverage_Analysis/out_data/General_LCO_effectiveCov.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[b]{0.62\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{../../project/Coverage_Analysis/out_data/Inertial_LCO_effectiveCov.png}
     \end{subfigure}      
	 \\
     \begin{subfigure}[b]{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{../../project/Coverage_Analysis/out_data/Visual_LCO_effectiveCov.png}
     \end{subfigure}
     \hfill
        \caption{Effective Coverage Dynamic Range - Least Cost}
        \label{fig:covDR_LCO}
\end{figure}

==> figs/covDR_LEO.tex <==
% Correlation plots
\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.31\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{../../project/Coverage_Analysis/out_data/General_LEO_effectiveCov.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[b]{0.62\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{../../project/Coverage_Analysis/out_data/Inertial_LEO_effectiveCov.png}
     \end{subfigure}      
	 \\
     \begin{subfigure}[b]{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{../../project/Coverage_Analysis/out_data/Visual_LEO_effectiveCov.png}
     \end{subfigure}
     \hfill
        \caption{Effective Coverage Dynamic Range - Least Experiments}
        \label{fig:covDR_LEO}
\end{figure}

==> figs/eff_cov_desc.tex <==
\begin{figure}[!tp]
     \centering
         \includegraphics[width=\columnwidth]{img/eff_cov_BD.png}
        \caption{A Flowchart of Effective Coverage Calculation}
        \label{fig:eff_cov}
\end{figure}

==> figs/greedy_desc.tex <==
\begin{figure}[!tp]
     \centering
         \includegraphics[width=0.8\columnwidth]{img/greedy_BD.png}
        \caption{A Flowchart of the Greedy-based Optimization}
        \label{fig:greedy_algo}
\end{figure}

==> figs/seqFullCov_LCO.tex <==
% Correlation plots
\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.31\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{../../project/Coverage_Analysis/out_data/General_LCO_SeqToFullCoverage.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[b]{0.62\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{../../project/Coverage_Analysis/out_data/Inertial_LCO_SeqToFullCoverage.png}
     \end{subfigure}      
	 \\
     \begin{subfigure}[b]{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{../../project/Coverage_Analysis/out_data/Visual_LCO_SeqToFullCoverage.png}
     \end{subfigure}
     \hfill
        \caption{No. of Sequence to Full Coverage - Least Cost}
        \label{fig:fullCov_LCO}
\end{figure}

==> figs/seqFullCov_LEO.tex <==
% Correlation plots
\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.31\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{../../project/Coverage_Analysis/out_data/General_LEO_SeqToFullCoverage.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[b]{0.62\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{../../project/Coverage_Analysis/out_data/Inertial_LEO_SeqToFullCoverage.png}
     \end{subfigure}      
	 \\
     \begin{subfigure}[b]{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{../../project/Coverage_Analysis/out_data/Visual_LEO_SeqToFullCoverage.png}
     \end{subfigure}
     \hfill
        \caption{No. of Sequence to Full Coverage - Least Experiments}
        \label{fig:fullCov_LEO}
\end{figure}

==> greedy_material.tex <==
\subsection{Greedy-Based Optimization}
\textit{Greedy Algorithms} is a methodology for solving optimization problems that depends on selecting the best available options at the time of decision \cite{cormen2022introduction}. The algorithm does not allow rolling back a taken decision based on observed better alternatives. Thus, it can yield a sub-optimal or even a non-optimal solution upon termination due to its reliance on achieving local-optimality.
\input{algos/greedy_leastExp.tex}

As shown in Algorithm \ref{greedy_algo}, the first and most fundamental step of the greedy-based approaches is defining a heuristic by which all candidate inputs to the algorithm are sorted. The heuristic can change based on the target objective of the algorithm as we will illustrate in the following section.

\subsection{Minimization of the Number of Experiments/Sequences}
The context switching between experiments in the testing environment of SLAM can consume a lot of time specially when each sequences has its own configurations that needs to be set prior to running the algorithm either manually or automatically using configuration files. In this segment of the proposed work, we assume a constant cost for all of the available data sequences.

In greedy-based approaches, to achieve the minimum number of experiments, a heuristic must be selected to represent each data sequence. In our case, the previously defined \textit{Absolute Total Coverage} $ADC_{\mathcal{C}_k}$, given in \ref{equ:ATC}, is selected for that purpose.

\subsection{Minimization of the Total Coverage Cost}
Due to the difference in sequence sizes, the context switching between experiments may not be the dominating factor in determining the total experiments time. Rather, the size of each sequence and the amount of coverage they provide would be of a much greater importance. 

In greedy-based approaches, the sorting heuristic is selected to be the coverage cost $\mathcal{COV}_{cost}$ defined in \ref{cov_cost_equ}. The sorting objective is adjusted accordingly and the algorithm \ref{greedy_algo} operates similarly.

==> methodology_old.tex <==
\subsection{Greedy-Based Optimization}
Historically, the problem of finding the optimal subset of intervals to match a target range was solved using greedy-based approaches \cite{prolubnikov2015set}, due to their simplicity, resulting in an acceptable sub-optimal solution in a polynomial time.

\textit{Greedy algorithms} is a methodology for solving optimization problems that depends on selecting the best available options at the time of decision \cite{cormen2022introduction}. The algorithm does not allow rolling back a taken decision based on observed better alternatives. Thus, it can yield a sub-optimal or even a non-optimal solution upon termination due to its reliance on achieving local-optimality. As shown in Figure \ref{fig:greedy_algo}, the first and most fundamental step of the greedy-based approaches is defining a heuristic by which all candidate inputs are sorted. The heuristic can change based on the target objective of the algorithm.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{figs/DP_desc.tex}
\subsection{Tabulation-Based Dynamic Programming Optimization}


==> problem_def_old.tex <==
\section{Problem Definition}
\label{sec:problem_def}
The existence of redundancy within and between datasets leads to unreliable experimental setup, where evaluation objectives are not guaranteed to be addressed. This gives rise to the need to select a subset of evaluation sequences from available datasets that reaches similar coverage levels for certain quantifiable objective. For instance, we seek to answer whether the full KITTI dataset is needed to test for illumination changes or not. If not, which sequences in KITTI dataset are representing of the coverage level achieved by the full dataset. 

\subsection{Dataset and Characterization Representation}
Each dataset is divided into $q$ sequences $Q_{1..q}$ each representing a single data acquisition and recording session. Dataset sequences can be characterized by characterization metrics, where a set of values are generated for each metric \cite{ali2022we}. Accordingly, each characterization metric produces a set of $c$ values $\mathcal{C}_{1..c}$, where $c$ matches the number of measurements in a sequence. This vector is considered a random variable with a bounded range. \textit{Dynamic range coverage $\mathcal{COV}$} is a measure of the range of characterization values $\mathcal{C}_{1..c}$ tested. Thus, for a given characterization metric, a sequence or dataset can be considered a continuous random variable \cite{rice2006mathematical}, and can be represented by their measured boundary values deduced from the minimum and maximum measured values: $C_{min}$ and $C_{max}$. 
For example, KITTI provides 22 sequences of data ($q=22$), one of these sequence is seq.09 where each it consists of 1591 measurement(i.e. images). Characterizing the brightness of this sequence produces 1591 value corresponding to each image in the sequence. In this case, $C_{min}$ and $C_{max}$ represents the least and most bright images in the sequence respectively. 

\subsection{Dynamic Range Coverage Parameters}
Given the abstraction of each characterized sequence as a continuous random variable, one can represent in the form of the range $[C_{min}, C_{max}]$. Thus, the simplest method to calculate the magnitude of the dynamic range coverage of a single data sequence (e.g. KITTI seq.09) for a one characterization metric (e.g. brightness) is by subtracting the range bounds. 
\begin{equation}
\label{equ:ATC}
Coverage\;Magnitude =  C_{max} - C_{min}
\end{equation}

To acquire the total dynamic range coverage of a set of sequences (e.g. the full KITTI dataset), dynamic range coverage magnitudes must be aggregated taking into consideration intersections and discontinuity regions. Figure \ref{fig:eff_cov} provides an illustration of the process.
\input{figs/eff_cov_desc.tex}

To achieve a certain level of coverage $\mathcal{COV}$, validation sequences are chosen from either a single dataset or multiple datasets. We define the cost of achieving coverage $\mathcal{COV}_{cost}$ as the number of processed measurements (e.g. images) by SLAM scaled by the dynamic range of a characterization metric. For instance, the cost of achieving full coverage of brightness values using KITTI dataset can be calculated by scaling the total number of images of all KITTI sequences by the measured dynamic range. 

Additionally, the percentage of coverage $\mathcal{COV}_{\%}$ is defined as the ratio of the achieved dynamic range coverage by a certain method (e.g. a certain dataset, or the outcome of our proposed algorithm) divided by the target dynamic range coverage (e.g. the coverage of all dataset combined for a certain characterization metric).

Finally, we define the number of sequences required to achieve full coverage percentage ($\mathcal{COV}_{\%} = 100\%$) to be $\mathcal{COV}_{\mathcal{Q}}$.
\input{figs/greedy_desc.tex}
\subsection{Minimizing Single-Objective SLAM Evaluation Footprint}
In order to reduce the footprint of SLAM evaluation while achieving a certain level of dynamic range coverage over an objective characterization metric, we need to either reduce the number of sequences tested $\mathcal{COV}_{\mathcal{Q}}$ or reduce the coverage cost $\mathcal{COV}_{cost}$ of the evaluation subset. For instance, using KITTI, EuroC-MAV, and TUM-VI combined requires the execution of a total of 61 experiment, where each experiment is done on one sequence. The optimal subset will have less sequences with same coverage range.

The former objective is achieved by finding the least number of validation sequences $\widetilde{q}$,  to achieve $100\%$ of the target dynamic range coverage, which is given by:
\begin{equation}
\arg \min_{q} \quad \sum\limits_{i=1}^{\widetilde{q}} \mathds{1} (\left.\mathcal{Q}_i\right|_{\mathcal{C}}) \quad
\textrm{s.t.} \quad  \mathcal{COV}_{\%} = 100\%\; \&\; \widetilde{q} \leq q
\end{equation}
where $\mathcal{Q}_i$ is an sequence in the optimal subset, $\mathcal{C}$ is the characterization metric under investigation, and $q$ is the size of the optimal subset. 

The latter objective is achieved by finding the set of validation sequences that achieves $100\%$ of the target dynamic range coverage, while minimizing the total cost of coverage by picking the subset of sequences that minimizes the number of measurements (e.g. images) processed to achieve the target coverage, i.e., 

\begin{align}
\arg \min_{m_i} &\quad {\sum\limits_{i=0}^{\widetilde{q}} (\left.m_i\right|_{\mathcal{C}}) }/{total\;coverage} \nonumber \\
\textrm{s.t.} &\quad  \mathcal{COV}_{\%} = 100\%\; \&\; \widetilde{q} \leq q
\end{align}

where $m_i$ is the number of measurements (e.g. images) in a selected data sequence, and $\mathcal{C}$ is the characterization metric under investigation.


==> results_old.tex <==
\input{tables/summary_results.tex}
\input{figs/agg_results.tex} 
Three datasets, KITTI \cite{geiger2012we}, EuroC-MAV \cite{burri2016euroc}, and TUM-VI \cite{schubert2018tum},  and their characterizations were used to demonstrate the performance of the proposed method. When combined, they provide a total of 61 sequences. The corresponding combined dynamic range is used as the target coverage range ($100\%$ coverage). Moreover, the coverage analysis parameters were calculated for each dataset and for the three combined, which was selected as our baseline. Finally, the coverage analysis parameters were calculated on the results of the proposed algorithm when run with the two optimization objectives.

\subsection{Single-Objective SLAM Coverage}
Metric-level results were averaged for each characterization category to provide an aggregated result valid for comparison of different objectives. Figure \ref{fig:agg_results} provides a comparison of the coverage cost, coverage percentage, and the number of sequences to full coverage for different categories. Additionally, the results were tabulated in Table \ref{tab:summary_res}.

As shown in Figure \ref{fig:agg_results}, using a single dataset is not sufficient to reach full coverage. More specifically, we can observe the superiority of the TUM-VI dataset in coverage of both the general and the visual characterization metrics, while being out-performed in terms of inertial characterization metrics by EuroC-MAV dataset.

Applying DP optimization showed that, full coverage can be achieved by selecting a hybrid sequence mix from the three available datasets. For instance, the reduction of the coverage cost with least cost optimization was: 9.1x, 6.4x, 28.2x for the general, inertial and visual characterization metrics categories respectively. This highlights a high level of redundancy in the tested datasets.

The number of sequences associated with each characterization metric category was reduced as well to the levels of 2.6, 1.58, 2.81 sequences to achieve full coverage compared to 44.5, 18.53, 42.14 sequences when using the baseline. This reduction can also be compared to the conventional testing methodology used in the SLAM literature of running all the sequences of the three datasets (a total of 61 sequence). The results shown suggests that running the aforementioned and limited number of sequences can achieve the same coverage levels of running all the sequences of the three datasets combined. 

\input{figs/joint_LEO.tex}
\subsection{Extending to Multi-Objective SLAM Coverage}
The proposed method can be extended to deduce an optimized list of sequences to achieve coverage over multiple characterization metrics. A brute-force approach is to perform a set union operation on the resulting optimal coverage sets of each contributing metric. The results of this process are presented in Figure \ref{fig:joint_coverage}. The experiment incorporates increasing the number of characterization metric mentioned in \cite{ali2022we} gradually and calculating the number of sequences needed to achieve full coverage over incorporated metrics. The experiment shows the superiority of the DP solution and its ability to reduce the validation sequence subset by almost 30\%.

\subsection{SLAM Performance Under Reduced Evaluation Set}
\input{tables/ATE_analysis_tab.tex}
%\input{figs/ATE_analysis.tex}
Achieving robustness is tightly coupled with linking SLAM performance to the associated dynamic range \cite{prorok2021beyond}. Thus, we evaluated the ATE properties of two SLAM algorithms which are: ORB-SLAM3 \cite{campos2021orb} and VINS-Mono \cite{qin2018vins} on the complete TUM-VI dataset and the optimized TUM-VI dataset taking into consideration the multi-objective coverage of 73 characterization metrics. The results presented in Table \ref{tab:ATE_analysis_tab} show that, the SLAM ATE properties are the same after reducing the evaluation footprint by 15\%, and is almost the same after a 30\% reduction using only inertial metrics. 
To measure the significance of the selected subset of sequences in describing the ATE properties of a SLAM algorithm, the DP-optimized subset was compared to the random selection of sequences of the same size. Due to the unbalanced distribution of the ATE values, Wasserstein distance \cite{panaretos2019statistical} is used to measure the similarity between the probability distribution of the reduced TUM-VI subset and a randomly selected TUM-VI subset. The experiment included increasing the subset size until the full TUM-VI dataset is included, and comparing the 24 sequence cut-off with the DP-based results as shown in Fig. \ref{fig:ATE_rand_fig}. The experiment outcomes were averaged over 2000 iterations. Calculating the probability of producing the same DP results from random experiments showed that, DP subset is closer in distance to the original subset with distance less than 45\% of its random counterpart. Additionally, the probability of producing the same DP outcomes randomly is very improbable with a probability approaching zero as shown in Table \ref{tab:ATE_rand_tab}. The results hold true for both ORB-SLAM3 and VINS-Mono.

\input{figs/ATE_rand_test.tex}
\input{tables/ATE_rand_tab.tex}

==> tables/ATE_analysis_tab.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[!tp]
\caption{ATE Properties with Reduced Evaluation Footprint for All, general (G), inertial (I), and Visual (V) Characterization Metrics}
\label{tab:ATE_analysis_tab}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lcccc|ccc@{}}
\cmidrule(l){3-8}
\textbf{} &
  \multicolumn{1}{l}{} &
  \multicolumn{3}{c|}{\textbf{ORB-SLAM3}} &
  \multicolumn{3}{c}{\textbf{VINS-Mono}} \\ \cmidrule(l){2-8} 
\multicolumn{1}{l|}{\textbf{Eval. Setup}} &
  \multicolumn{1}{c|}{\textbf{\# Seq}} &
  \textbf{$\mu$} &
  \textbf{Med} &
  \textbf{$\sigma$} &
  \textbf{$\mu$} &
  \textbf{Med} &
  \textbf{$\sigma$} \\ \midrule
\multicolumn{1}{l|}{\textbf{Full TUM-VI}} &
  \multicolumn{1}{c|}{\textbf{28}} &
  \textbf{5.56} &
  \textbf{0.48} &
  \textbf{11.62} &
  \textbf{23.29} &
  \textbf{0.89} &
  \textbf{43.20} \\ \midrule
\multicolumn{1}{l|}{\textbf{Reduced TUM-VI (All)}} &
  \multicolumn{1}{c|}{\textbf{24}} &
  \textbf{5.94} &
  \textbf{0.44} &
  \textbf{12.38} &
  \textbf{23.45} &
  \textbf{0.89} &
  \textbf{44.39} \\ \midrule
\multicolumn{1}{l|}{Reduced TUM-VI (G)} &
  \multicolumn{1}{c|}{6} &
  2.99 &
  1.17 &
  3.78 &
  44.83 &
  1.94 &
  61.73 \\
\multicolumn{1}{l|}{\textbf{Reduced TUM-VI (I)}} &
  \multicolumn{1}{c|}{\textbf{19}} &
  \textbf{7.44} &
  \textbf{0.47} &
  \textbf{13.52} &
  \textbf{29.43} &
  \textbf{1.56} &
  \textbf{48.14} \\
\multicolumn{1}{l|}{\textbf{Reduced TUM-VI (V)}} &
  \multicolumn{1}{c|}{\textbf{24}} &
  \textbf{5.94} &
  \textbf{0.44} &
  \textbf{12.38} &
  \textbf{23.45} &
  \textbf{0.89} &
  \textbf{44.39} \\ \bottomrule
\end{tabular}
}
\end{table}

==> tables/ATE_rand_tab.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\caption{Wasserstine Distance of a randomly selected vs. DP-selected sequence sub-set}
\label{tab:ATE_rand_tab}
\begin{tabular}{@{}lccc@{}}
\toprule
\multicolumn{1}{l|}{\textbf{Eval. Setup}} & \multicolumn{1}{c|}{\textbf{\# Seq}} & \textbf{ORB-SLAM3}        & \textbf{VINS-Mono}         \\ \midrule
\multicolumn{1}{l|}{Random Sub-set}      & \multicolumn{1}{c|}{24} & 0.9042067 & 3.2687920 \\
\multicolumn{1}{l|}{DP-Selected Sub-set} & \multicolumn{1}{c|}{24} & 0.4923214 & 1.7422619 \\ \midrule
\textbf{DP vs. Random}                    & \multicolumn{1}{l}{\textbf{}}       & \textbf{45.5\% (P=0.003)} & \textbf{46.7\% (P=0.0015)} \\ \cmidrule(r){1-1} \cmidrule(l){3-4} 
\end{tabular}
\end{table}
